Expanding Horizons in HCI Research Through LLM-Driven Qualitative Analysis

How would research be like if we still needed to "send" papers typed with a typewriter? Our life and research environment have continually evolved, often accompanied by controversial opinions about new methodologies. In this paper, we embrace this change by introducing a new approach to qualitative analysis in HCI using Large Language Models (LLMs). We detail a method that uses LLMs for qualitative data analysis and present a quantitative framework using SBART cosine similarity for performance evaluation. Our findings indicate that LLMs not only match the efficacy of traditional analysis methods but also offer unique insights. Through a novel dataset and benchmark, we explore LLMs' characteristics in HCI research, suggesting potential avenues for further exploration and application in the field.

==> Section/1_Introduction.tex <==
Qualitative research demands substantial effort, primarily due to the rigorous processes involved in coding, categorizing and interpreting voluminous data~\cite{Guetterman2018,Kaufmann2020}. Over the years, efforts have been made to automate these processes by leveraging technologies such as Natural Language Processing (NLP) in an attempt to alleviate the load. In conventional practice, NLP has been utilized in qualitative analysis to facilitate tasks such as creating codebooks or categorizing data, which are essential in the thesis writing process~\cite{Abram2020}.

A noticeable shift in focus towards large language models (LLMs) occurred with the advent of ChatGPT in 2022, where research began exploring their potential in aiding qualitative analysis, notably in tasks such as codebook categorization~\cite{Tai2023, Bano2023}. However, these studies primarily employ NLP and LLMs as auxiliary tools, assisting humans in data compilation, leaving data interpretation and discussion largely untouched, indicating room for automation.2023

LLMs, by their very nature, excel at language processing, particularly in rendering linguistic feedback on substantial language data [Cite recent studies on LLM capabilities]. Given the dramatic advancements in LLM technology, it is plausible that LLMs could go beyond merely processing large language data and categorizing them into statistically amenable formats. In fact, Byun et al.(2023) proposed using LLMs to directly generate discussions from raw qualitative analysis data. However, their results weren't quantitatively evaluated, making it difficult to determine the effectiveness of their method. ~\cite{Byun2023}.

In this paper, we propose a method for performing qualitative analysis using LLMs, and we offer a quantitative evaluation of the output using a dataset comprising eight published papers from the CHI and HCI domains that conducted qualitative analysis, along with their raw interview data. It leads to two contributions,

\begin{itemize}
\item contribution a
\item contribution b.
\end{itemize}

